Computing Rule-Based Explanations by Leveraging Counterfactuals

Sophisticated machine models are increasingly used for high-stakes decisions in everyday life. There is an urgent need to develop effective explanation techniques for such automated decisions. Rule-Based Explanations have been proposed for high-stake decisions like loan applications, because they increase the users' trust in the decision. However, rule-based explanations are very inefficient to compute, and existing systems sacrifice their quality in order to achieve reasonable performance. We propose a novel approach to compute rule-based explanations, by using a different type of explanation, Counterfactual Explanations, for which several efficient systems have already been developed. We prove a Duality Theorem, showing that rule-based and counterfactual-based explanations are dual to each other, then use this observation to develop an efficient algorithm for computing rule-based explanations, which uses the counterfactual-based explanation as an oracle. We conduct extensive experiments showing that our system computes rule-based explanations of higher quality, and with the same or better performance, than two previous systems, MinSetCover and Anchor.

==> sections/Experiments/End_End.tex <==

\begin{table*}[htbp!]
\centering
 \begin{tabular}{|c|c|c|c|c|c|c|c|} 
 \hline
    & x & Genetic Rule & GR with GeCo & GeCo Greedy & Anchor & Set Cover & Viol. \\ 
 \hline\hline ExternalRiskEstimate& 59&Decrease&Decrease&Decrease&Decrease& &81\\
 \hline MSinceMostRecentTradeOpen& -8& && & Decrease& & \\
 \hline AverageMInFile&82&  &  && Increase& & \\
 \hline NumSatisfactoryTrades&20  &  &  &&  Fixed&Decrease& \\
 \hline PercentTradesNeverDelq&78&  Decrease&Decrease&  Decrease&  Decrease&&96 \\
  \hline MaxDelq2PublicRecLast12M&4&  Decrease&&  &  Decrease& & \\
  \hline MaxDelqEver&2&  &  &&  Decrease& & \\
  \hline NumTotalTrades&27&  &  &&  Fixed& & \\
   \hline NumTradesOpeninLast12M&1&  &  &&  Fixed& & \\
   \hline MSinceMostRecentInqexcl7days&4&  &  & & Increase& & \\
   \hline NetFractionRevolvingBurden&98&  Increase& Increase&  Increase&  Increase& &49 \\
   \hline NetFractionInstallBurden&84&  &  &&  Increase& & \\
   \hline NumRevolvingTradesWBalance&2&  &  &&  Decrease& & \\
   \hline NumBank2NatlTradesWHighUtilization&-8&  Decrease&  &&  Decrease& & \\
   \hline PercentTradesWBalance&100&  &  &&  Increase&Decrease & \\
 \hline
\end{tabular}
\vspace{1.2mm}
 \caption{Examples of Rule Explanations by Genetic Rule, Genetic Rule with GeCo, GeCo Greedy, Anchor, Set Cover, Violation Counterfactual for Set Cover for one instance in Fico (presenting selected features)}
 \label{tab:end_end}
\end{table*}

\subsection{End-to-end Example}
We consider one specific instance in the Fico dataset that is classified as "undesired" and illustrate the rule explanations generated for each considered system.


Table \ref{tab:end_end} presents the instance $x$ and the rule explanations generated by Genetic Rule, Genetic Rule with GeCo, GeCo Greedy, Anchor, and Set Cover. The rule explanation from Set Cover is failed in the feature space verification, so we also present the counterfactual violation to it.

For this instance, Genetic Rule with GeCo and GeCo Greedy return the same rule explanation with a cardinality of 3 that is verified in both dataset and feature space and has no redundant components. Genetic Rule returns a rule explanation with the cardinality of 5 which is verified in both dataset and feature space but has two redundant components for MaxDelq2PublicRecLast12M and NumBank2Natl-\\TradesWHighUtilization. Anchor surprisingly returns a rule explanation with the cardinality of 15. It is verified in both dataset and feature space but has 12 redundant components. Set Cover returns a rule explanation with the cardinality of 2, but is failed in the feature space verification. We can find a counterfactual with 3 feature changes and none of these features are restricted by the rule.
